SealQA: Raising the Bar for Reasoning in Search-Augmented Language Models

We introduce SealQA, a new challenge benchmark for evaluating SEarch-Augmented Language models on fact-seeking questions where web search yields conflicting, noisy, or unhelpful results. SealQA comes in three flavors: (1) Seal-0 (main) and (2) Seal-Hard, which assess factual accuracy and reasoning capabilities, with Seal-0 focusing on the most challenging questions where chat models (e.g., GPT-4.1) typically achieve near-zero accuracy; and (3) LongSeal, which extends SealQA to test long-context, multi-document reasoning in "needle-in-a-haystack" settings. Our evaluation reveals critical limitations in current models: Even frontier LLMs perform poorly across all SealQA flavors. On Seal-0, frontier agentic models equipped with tools like o3 and o4-mini achieve only 17.1% and 6.3% accuracy, respectively, at their best reasoning efforts. We find that advanced reasoning models such as DeepSeek-R1-671B and o3-mini are highly vulnerable to noisy search results. Notably, increasing test-time compute does not yield reliable gains across o3-mini, o4-mini, and o3, with performance often plateauing or even declining early. Additionally, while recent models are less affected by the "lost-in-the-middle" issue, they still fail to reliably identify relevant documents in LongSeal when faced with numerous distractors. To facilitate future work, we release SealQA at huggingface.co/datasets/vtllms/sealqa.

==> tables/results_combine.tex <==
\begin{table*}[t]
\centering

\begin{minipage}[t]{0.48\textwidth}
\centering
\caption{\sscnoxsp{LLMs} struggle with questions that involve recent information on \sscnoxsp{Seal-Hard}.}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\ssc{w/o search}} & \multicolumn{3}{c}{\ssc{w/ search}} \\ \cline{2-7}
 & \ssc{$<$ 2024} & \ssc{2024} & \ssc{2025} & \ssc{$<$ 2024} & \ssc{2024} & \ssc{2025} \\
\midrule
% -------- closed‑source header in yellow --------
\ssc{GPT-4.1}          & 23.5 & 6.1 & 0.0 & 25.5$^\dagger$ & 20.4$^\dagger$ & 7.1$^\dagger$ \\
\ssc{o3-mini-high}          & 20.5 & 2.6 & 1.4 & 14.4 & 12.8 & 4.3 \\
\ssc{o3-high}         &   –  &  –  &  –  & 45.9$^\dagger$ & 15.4$^\dagger$ & 14.5$^\dagger$ \\
\ssc{Llama-4‑Scout}                   &  8.7 & 4.1 & 0.0 &  7.4 &  6.1 & 1.8 \\
\ssc{DeepSeek-R1}                    & 35.6 & 8.2 & 0.0 & 14.8 &  6.1 & 5.4 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{table:results_effective_year}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\caption{On \sscnoxsp{Seal-Hard}, performance degrades more when search results are uniformly unhelpful than when they contain conflicting answers.}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{2}{c}{\ssc{w/o search}} &
\multicolumn{2}{c}{\ssc{w/ search}} \\ \cline{2-5}
 & \ssc{unhelpful} & \ssc{conflict.} & \ssc{unhelpful} & \ssc{conflict.} \\
\midrule
\ssc{GPT-4.1}          & 14.5 & 15.3 & 18.2$^\dagger$ & 22.2$^\dagger$ \\
\ssc{o3-mini-high}          & 10.9 & 13.9 & 8.2 & 13.9 \\
\ssc{o3-high}         &   –  &   –  & 30.0$^\dagger$ & 34.7$^\dagger$ \\
\ssc{Llama-4‑Scout}                   & 3.6 &  7.6 &  4.5 &  6.9 \\
\ssc{DeepSeek-R1}                    &20.9 & 23.6 &  9.1 & 12.5 \\
\bottomrule
\end{tabular}
\end{adjustbox}
%\vspace{-3mm}
\label{table:results_search_quality}
\end{minipage}
\end{table*}
